TIPS: Threat Sharing Information Platform for Enhanced Security

There is an increasing need to share threat information for the prevention of widespread cyber-attacks. While threat-related information sharing can be conducted through traditional information exchange methods, such as email communications etc., these methods are often weak in terms of their trustworthiness and privacy. Additionally, the absence of a trust infrastructure between different information-sharing domains also poses significant challenges. These challenges include redactment of information, the Right-to-be-forgotten, and access control to the information-sharing elements. These access issues could be related to time bounds, the trusted deletion of data, and the location of accesses. This paper presents an abstraction of a trusted information-sharing process which integrates Attribute-Based Encryption (ABE), Homomorphic Encryption (HE) and Zero Knowledge Proof (ZKP) integrated into a permissioned ledger, specifically Hyperledger Fabric (HLF). It then provides a protocol exchange between two threat-sharing agents that share encrypted messages through a trusted channel. This trusted channel can only be accessed by those trusted in the sharing and could be enabled for each data-sharing element or set up for long-term sharing.

==> glos.tex <==
\newglossaryentry{GDPR}
{
name=GDPR (General Data Protection Regulation),
description={An EU regulation for data protection}
}


\newglossaryentry{IPFS}
{
name=IPFS (Interplanetary File System),
description={A distributed file system which uses a CID to link to a file}
}

\newglossaryentry{EMR}
{
name=EMR (Electronic Medical Record),
description={An electronic version of a patient health record}
}

\newglossaryentry{WHO}
{
name=WHO (World Health Organisation),
description={A United Nations organisation for public health on an international level}
}

\newglossaryentry{RTBF}
{
name=RTBF (Right-to-be-forgotten),
description={A core part of GPDR, and which defines that a citizen has the right to have their personal data removed from Internet searches}
}

\newglossaryentry{CDS}
{
name=CDS (Clinical Decision Support),
description={A health care system which allows improved clinical outcomes}
}

\newglossaryentry{KYC}
{
name=KYC (Know Your Customer),
description={A method which aims to gather key details about customers and that relate to their identity}
}

\newglossaryentry{HIPAA}
{
name=HIPAA (Health Insurance Portability and Accountability Act),
description={A US health regulation to protect health care information}
}

\newglossaryentry{Homomorphic Encryption}
{
name=HE (Homomorphic Encryption),
description={A method of public key encryption which allows data to be encrypted with a public key and then can be processed with the encrypted form. An associated private key will then decrypt the result}
}

\newglossaryentry{ZKP}
{
name=ZKP (Zero Knowledge Proof),
description={A method which protects the privacy of data, and where there is a proof of the knowledge of the data}
}

\newglossaryentry{RPM}
{
name=RPM (Remote Patient Monitoring,
description={A method of providing trusted monitoring of patients}
}
\newglossaryentry{Hyperledger}
{
name=Hyperledger (IBM Hyperledger,
description={An open-source permissioned ledger and supported by the Hyperledger Foundation.}
}

\newglossaryentry{Ethereum}
{
name=Ethereum,
description={A permissionless ledger that implements smart contracts}
}

\newglossaryentry{C3ISP}
{
name=C3ISP,
description={Cyber threat intelligence (CTI) has been proposed to achieve cyber threat information sharing between organisations}
}

\newglossaryentry{DIDs}
{
name=DIDs,
description={A decentralised Identifier}
}



\newglossaryentry{SSI}
{
name=SSI,
description={Self-sovereign identity}
}


\newglossaryentry{CTI}
{
name=CTI,
description={Cyber Threat Information}
}


\newglossaryentry{STIX}
{
name=STIX,
description={Structured Threat Information CybereXpression (STIX)}
}

\newglossaryentry{TAXII}
{
name=TAXII,
description={Trusted Automated eXchange of Indicator Information (TAXII)}
}

\newglossaryentry{ABE}
{
name=ABE,
description={Attributed-based encryption is a method that allows a policy to be defined for the encryption and decryption process, such as locking it down to specific time periods or for the location of the access.}
}

\newglossaryentry{FHE}
{
name=FHE,
description={Fully Homomorphic Encryption allows for every mathematical operation to be conducted on encrypted data. }
}















